DIB-R++: Learning to Predict Lighting and Material with a Hybrid Differentiable Renderer

We consider the challenging problem of predicting intrinsic object properties from a single image by exploiting differentiable renderers. Many previous learning-based approaches for inverse graphics adopt rasterization-based renderers and assume naive lighting and material models, which often fail to account for non-Lambertian, specular reflections commonly observed in the wild. In this work, we propose DIBR++, a hybrid differentiable renderer which supports these photorealistic effects by combining rasterization and ray-tracing, taking the advantage of their respective strengths -- speed and realism. Our renderer incorporates environmental lighting and spatially-varying material models to efficiently approximate light transport, either through direct estimation or via spherical basis functions. Compared to more advanced physics-based differentiable renderers leveraging path tracing, DIBR++ is highly performant due to its compact and expressive shading model, which enables easy integration with learning frameworks for geometry, reflectance and lighting prediction from a single image without requiring any ground-truth. We experimentally demonstrate that our approach achieves superior material and lighting disentanglement on synthetic and real data compared to existing rasterization-based approaches and showcase several artistic applications including material editing and relighting.

==> doc/fig_abllightnum.tex <==

\begin{figure}
	\vspace*{-0cm}
	\begin{center}
		\setlength{\tabcolsep}{1pt}
		\setlength{\fboxrule}{1pt}
		\begin{tabular}{c}
			\begin{tabular}{cccccccccccc}
				&
				\multicolumn{1}{c}{ \scriptsize Input } &
				\multicolumn{1}{c}{ \scriptsize GT albedo } & \multicolumn{2}{c}{\scriptsize GT lighting (envmap)} &
				\multicolumn{2}{c}{\scriptsize Pred. light ({\sgshort})} &
				\multicolumn{1}{c}{\scriptsize Texture} &
				\multicolumn{2}{c}{\scriptsize Pred. albedo} &
				\multicolumn{2}{c}{\scriptsize Re-rendered (with light)}
				\\
				\rotatebox{90}{\scriptsize GT }
				& &  & &  & & & &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-4-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-4-00.png}} 
				\\
				\rotatebox{90}{\scriptsize 4 $\sg_l$}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/4/real_0160002-2-00.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/4/160002.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/4/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/4/real_0160002-3-01.png}} 
				\\
				\rotatebox{90}{\scriptsize 8 $\sg_l$}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/8/real_0160002-2-00.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/8/160002.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/8/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/8/real_0160002-3-01.png}} 
				\\
				\rotatebox{90}{\scriptsize 16 $\sg_l$}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/16/real_0160002-2-00.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/16/160002.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/16/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/16/real_0160002-3-01.png}} 
				\\
				\rotatebox{90}{\scriptsize 32 $\sg_l$}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-2-00.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/160002.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/9_abl_numberofsg/1/32/real_0160002-3-01.png}} 
				
			\end{tabular}
		\end{tabular}
	\end{center}
	
	\caption{ \textbf{Ablation Study of Number of {\sgshort} Components.} As the number of {\sgshort} components increase, the predicted lighting is more and more similar to the GT lighting and the color of predicted texture becomes more and more visually uniform, which indicates better disentanglement.}
	\label{fig:abl_numberofsg}
	\vspace*{-0.0cm}
\end{figure}



==> doc/fig_ablloss.tex <==

\begin{figure}
	
	\begin{center}
		\setlength{\tabcolsep}{1pt}
		\setlength{\fboxrule}{1pt}
		\begin{tabular}{c}
			\begin{tabular}{cccccccccccc}
				&
				\multicolumn{1}{c}{ \scriptsize Input } &
				\multicolumn{1}{c}{ \scriptsize GT albedo } & \multicolumn{2}{c}{\scriptsize Pred. Shape} &
				\multicolumn{2}{c}{\scriptsize Pred. light ({\sgshort})} &
				\multicolumn{1}{c}{\scriptsize Texture} &
				\multicolumn{2}{c}{\scriptsize Pred. albedo} &
				\multicolumn{2}{c}{\scriptsize Re-rendered (with light)}
				\\
				\rotatebox{90}{\scriptsize $\loss_{im}$ \& $L_{msk}$}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/0.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/imloss/real_0160002-2-00.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/imloss/160002.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/imloss/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/imloss/real_0160002-3-01.png}} 
				\\
				\rotatebox{90}{\scriptsize + $\loss_{lap}$}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/1.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/implusreg/real_0160002-2-00.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusreg/160002.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/implusreg/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/implusreg/real_0160002-3-01.png}} 
				\\
				\rotatebox{90}{\scriptsize + $\loss_{per}$}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/2.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-2-00.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/160002.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/10_abl_loss/1/implusregpluspercept/real_0160002-3-01.png}} 
			\end{tabular}
		\end{tabular}
	\end{center}
	
	\caption{ \textbf{Ablation Study of Loss Terms.} Similar to ~\cite{zhang}, we also find $\loss_{\mathrm{lap}}$ regularizes the geometry to be smooth while $\loss_{\mathrm{per}}$ helps create high-frequency, detailed textures. }
	\label{fig:abl_loss}
	\vspace*{-0.0cm}
\end{figure}



\begin{figure}
	\hspace*{2cm}
	\begin{center}
		\setlength{\tabcolsep}{1pt}
		\setlength{\fboxrule}{1pt}
		\begin{tabular}{c}
			\begin{tabular}{ccccccccccccccc}
				\multicolumn{1}{c}{ \scriptsize Input } &
				\multicolumn{1}{c}{ \scriptsize GT albedo } & \multicolumn{1}{c}{\scriptsize Pred. albedo} & \multicolumn{2}{c}{\scriptsize GT lighting (envmap)} & 
				\multicolumn{2}{c}{\scriptsize Pred. light ({\sgshort})} & \multicolumn{4}{c}{\scriptsize Pred. material} &
				
				\multicolumn{2}{c}{\scriptsize GT specular} &
				\multicolumn{2}{c}{\scriptsize Pred. specular}
				\\
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160001-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160001-1-04.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160001-1-02.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160001-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160001-2-00.png}}  &
				\rotatebox{90}{\scriptsize $\rough_{gt}=0.242$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=1.0$} &
				\rotatebox{90}{\scriptsize $\rough_{pre}=0.228$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=0.108$} &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160001-4-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160001-3-01.png}} 
				\\
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160004-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160004-1-04.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160004-1-02.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160004-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160004-2-00.png}}  &
				\rotatebox{90}{\scriptsize $\rough_{gt}=0.389$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=1.0$} &
				\rotatebox{90}{\scriptsize $\rough_{pre}=0.270$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=0.046$} &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160004-4-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160004-3-01.png}} 
				\\
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160009-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160009-1-04.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160009-1-02.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160009-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160009-2-00.png}}  & 
				\rotatebox{90}{\scriptsize $\rough_{gt}=0.383$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=1.0$} &
				\rotatebox{90}{\scriptsize $\rough_{pre}=0.322$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=0.063$} &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160009-4-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160009-3-01.png}} 
				\\
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160011-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160011-1-04.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.09\linewidth]{fig_cameraready/fig_specular/1/32/real_0160011-1-02.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160011-2-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160011-2-00.png}}  &
				\rotatebox{90}{\scriptsize $\rough_{gt}=0.365$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=1.0$} &
				\rotatebox{90}{\scriptsize $\rough_{pre}=0.174$} &
				\rotatebox{90}{\scriptsize $\specAlbedo_{gt}=0.164$} &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160011-4-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.18\linewidth]{fig_cameraready/fig_specular/1/32/real_0160011-3-01.png}} 
				\\
			\end{tabular}
		\end{tabular}
	\end{center}
	
	\caption{ \textbf{Specular effect of {\sgshort} Shading.} We decompose the prediction into diffuse albedo, light and material parameters, then visualize the specular contribution in other views and compare with GT (last 4 columns). Although the predicted material parameters do not match GT, interestingly, the specular renderings align well with each other.}
	\label{fig:abl_speofsg}
	\vspace*{-0.0cm}
\end{figure}



==> doc/figalb_light.tex <==

\vspace*{-0cm}
\begin{figure}
	
	\begin{center}
		\setlength{\tabcolsep}{1pt}
		\setlength{\fboxrule}{1pt}
		\begin{tabular}{c}
			% \rotatebox{90}{\!\!\!\!\!\!\!\!\!\!{QR code}}~~~
			\begin{tabular}{ccccccccccc}
				&
				\multicolumn{1}{c}{ \scriptsize Input } &
				\multicolumn{1}{c}{ \scriptsize GT albedo } & \multicolumn{2}{c}{\scriptsize GT lighting (envmap)} &
				\multicolumn{2}{c}{\scriptsize {SG} + {\ourmodel}} &
				\multicolumn{2}{c}{\scriptsize {SG} + ~\cite{dibr}} &
				\multicolumn{2}{c}{\scriptsize {SH} + ~\cite{dibr}}
				\\
				&
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160011-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160011-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160011-2-01.png}}  &
				
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/sg/real_0160011-2-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160011-2-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160011-2-00.png}} 
				\\
				&
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160002-1-00.png}}  &  
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160002-1-04.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160002-2-01.png}}  &
				
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/sg/real_0160002-2-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160002-2-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160002-2-00.png}} 
			\end{tabular}
			\\
			\begin{tabular}{ccccccccccc}
				&
				\multicolumn{1}{c}{ \scriptsize Texture map } &
				\multicolumn{2}{c}{ \scriptsize Pred. albedo } & \multicolumn{2}{c}{\scriptsize Re-rendered (with light)} &
				\multicolumn{1}{c}{ \scriptsize Texture map } &
				\multicolumn{2}{c}{ \scriptsize Pred. albedo } & \multicolumn{2}{c}{\scriptsize Re-rendered (with light)}
				\\
				\rotatebox{90}{~~~~{GT}}
				&
				&  
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160011-4-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160011-4-00.png}}  &
				&
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160002-4-01.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160002-4-00.png}} 
				\\
				\rotatebox{90}{\scriptsize{SG+{\ourmodel}}}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/sg/160011.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/sg/real_0160011-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/sg/real_0160011-3-01.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/sg/160002.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/sg/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/sg/real_0160002-3-01.png}} 
				\\
				\rotatebox{90}{\scriptsize~~{SG+ ~\cite{dibr}}}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/160011.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160011-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160011-3-01.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/160002.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrsg/real_0160002-3-01.png}} 
				\\
				\rotatebox{90}{\scriptsize~~{SH+ ~\cite{dibr}}}
				&
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/160011.png}}  &  
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160011-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160011-3-01.png}}  &
				\multicolumn{1}{c}{\includegraphics[width=0.1\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/160002.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160002-3-00.png}}  &
				\multicolumn{2}{c}{\includegraphics[width=0.2\linewidth]{fig_cameraready/fig6_lightabl/1/iclrcolor/real_0160002-3-01.png}} 
			\end{tabular}
		\end{tabular}
	\end{center}
	
	\caption{ \textbf{Ablation Study of Shading Methods.} Even though we apply the same lighting representation to \cite{dibr}, due to the lack of specular transport suport, \cite{dibr} cannot perfectly disentangle the specular light from diffuse labedo. Its window and front cover still ``bake in'' white specular light. Moreover, the lighting is also blurry, as opposed to {\ourmodel}. This demonstrates the necessity of explicitly modelling advanced lighting effect in the renderer.}
	\label{fig:abl_sgshading}
	\vspace{10mm}
\end{figure}


==> doc/intro2.tex <==
\vspace{-5mm}
\section{Introduction}
\label{sec:intro}
\vspace{-3mm}

Inferring intrinsic 3D properties, including geometry, material and light, from a single image is a long-standing goal of computer vision \cite{barrow1978recovering}. Due to the severely under-constrained conditions, this task is . severe 

In recent years, differentiable rendering has shown great promise in estimating shape, reflectance and illumination from real photographs.
%Given the complex radiative coupling between objects in a scene, %---such as shadows and inter-reflections---inverting the forward rendering simulation process is fundamentally ill-posed. As such, effective disentanglement of geometry from material and lighting remain a challenging problem, especially in the single-view regime where the task is severly under-constrained.
%At their core, differentiable rendering techniques employ an analysis-by-synthesis approach where candidate images are first rendered in a forward pass and pixel losses are propagated to scene attributes in a backward pass through gradient-based optimization. 
Differentiable renderers have become natural candidates for learning-based inverse rendering applications, where image synthesis algorithms and neural networks can be jointly optimized to model physical aspects of objects from posed images, either by leveraging strong data priors  or by directly modeling the interactions between light and surfaces. %jun{Motivate from 3D content creation and talk about the problem in the beginning?}

Not all differentiable renderers are made equal. On the one hand, recent physics-based differentiable rendering techniques \cite{Li:2018:DMC, nimier2019mitsuba2, bangaru2020warpedsampling, NimierDavid2020Radiative, zhang2020psdr} try to model the full light transport with proper visibility gradients, but they tend to require careful initialization of scene parameters and typically exhibit high computational cost which limits their usage in larger end-to-end learning pipelines. On the other hand, performance-oriented differentiable renderers \cite{dibr, Laine2020diffrast, liu2019softras, kato2018renderer} trade physical accuracy for scalability and speed by approximating scene elements through neural representations or by employing simpler shading models. While this latter line of work has found some success in 3D scene reconstruction, the frequent assumptions of Lambertian-only surfaces and low-frequency lighting prevent them from modeling more complex specular transport commonly observed in the real world.

% material and direct illumination

%its methods usually fail in the single-image regime due to lack of visual cues for an efficient disentanglement of scene intrinsics.

%\jun{One-bounce ray tracing, no material, no background environment map?}

%In particular, rasterization-based \cite{opendr, chen2019dibrender, Laine2020diffrast} techniques provi

% to extract semantics from these images \cite{missing} or to for an effective decomposition. %This further imposes considerable constraints on the design space of such algorithms, where expressivity and computational efficiency must be properly balanced to achieve robustness.

%We follow this line of work here.

In this work, we  consider the problem of \textit{single-view 3D object reconstruction without any 3D supervision}. To this end, we propose DIB-R++, a hybrid differentiable renderer that combines rasterization and ray-tracing through an efficient deferred rendering framework. Our framework builds on top of DIB-R~\cite{dibr} and integrates physics-based lighting and material models to capture challenging non-Lambertian reflectance under unknown poses and illumination. Our method is versatile and supports both single-bounce ray-tracing and a spherical Gaussian representation for a compact approximation of direct illumination, allowing us to adapt and tune the shading model based on the radiometric complexity of the scene.
%exploits an interpretable GAN as an effective multi-view dataset generator to learn a strong prior to condition the input to our renderer \cite{zhang20style}.\jun{GAN? I think we should mainly talking about render in the intro? the application with ICLR paper can be left to application section} \joey{@Jun, the issue with not discussing this early on is that the paper feels underwhelming otherwise: SGs are not new (see NeRD, PhySG and other GFX papers like \cite{wang2009sg}), nor is DIB-R, so we really ought to be careful on how we present our method. The ``wow'' factor comes from this application, so I think we should put it up front?} \jun{I think we should differntiate learning-based inverse graphcs and optimization-based. In learning based method, we only see DIBR, Softras before, move to slack...}
% To augment the physical accuracy of our renderer, we are inspired by the recent success of spherical basis functions for modeling specular materials \cite{boss2020two, boss2020nerd, physg2020} and employ a spherical Gaussian representation to efficiently capture a wide variety of appearances and illumination configurations. In the case of near-mirror surfaces, our method also supports single-bounce ray-tracing.\jun{The story is we first have a framework xxx, and this framework support both single-bounce ray-tracing and SG, and they can be applied into different scenarios?}

% By introducing physics-based material and lighting models, our method captures a wide variety of appearances and illumination configurations while retaining a low computational cost. 

% More concretely, we propose to use spherical Gaussians to model specular materials and environment lighting, allowing for an efficient approximation of direct illumination. In the case of near-mirror surfaces, our method also supports single-bounce ray-tracing. 

We validate our technique on both synthetic and real images and 
%demonstrate the inherent ambiguity in jointly estimating scene parameters from few images.\jun{
demonstrate  superior performance on reconstructing realistic materials BRDFs and lighting configurations over prior rasterization-based methods. %We then show that conditioning our differentiable renderer with a GAN provides better disentanglement capability.
We then follow the setting proposed in Zhang \etal\cite{zhang20style} to %show that our {\ourmodel} can be conditioned on multi-view images generated from StyleGAN to accurately 
show that {\ourmodel} can reconstruct scene intrinsics also from real images without any 3D supervision. %, both quantitatively and visually. 
We further apply our framework to single-image appearance manipulation such as material editing and scene relighting.
%and demonstrate improved results over state-of-the-art techniques, both quantitatively and visually. 
%Our implementation will be made publicly available upon publication.
%\joey{We don't show quantitative results for those, so I would remove this sentence}


%More concretely, we introduce realistic BRDF and lighting models to the deferred shading pass to efficiently estimate direct illumination at the surface. We propose two shading techniques, namely ray-tracing or spherical Gaussians, and leverage their respective strengths to model view-dependent specular effects. We apply our technique to the problem of single-image reconstruction by training on a synthetic dataset to learn a strong prior on scene properties. We then show how we can leverage our differentiable deferred renderer to jointly predict shape and appearance from real-world images, allowing for several artistic applications such as scene relighting and material editing.

% In summary, our key contributions are:
% \begin{itemize}
%     \item Uno
%     \item Dos
%     \item Tres
% \end{itemize}

%Strong emphasis is placed on obtaining useful visibility gradients to facilitate shape inference via gradient descent.

